A Survey on Open-Source Edge Computing Simulators and Emulators: The Computing and Networking Convergence Perspective

Edge computing, with its low latency, dynamic scalability, and location awareness, along with the convergence of computing and communication paradigms, has been successfully applied in critical domains such as industrial IoT, smart healthcare, smart homes, and public safety. This paper provides a comprehensive survey of open-source edge computing simulators and emulators, presented in our GitHub repository (https://github.com/qijianpeng/awesome-edge-computing), emphasizing the convergence of computing and networking paradigms. By examining more than 40 tools, including CloudSim, NS-3, and others, we identify the strengths and limitations in simulating and emulating edge environments. This survey classifies these tools into three categories: packet-level, application-level, and emulators. Furthermore, we evaluate them across five dimensions, ranging from resource representation to resource utilization. The survey highlights the integration of different computing paradigms, packet processing capabilities, support for edge environments, user-defined metric interfaces, and scenario visualization. The findings aim to guide researchers in selecting appropriate tools for developing and validating advanced computing and networking technologies.

==> sect-others.tex <==
\section{Other Simulators}
\tablename~\ref{tab:compt-paradigms}
\section{Other Helpful Tools/Simulators}

\begin{table}
    \centering
    \caption{Other Helpful Tools/Simulators}
    \label{tab:compt-paradigms}
    \begin{tabular}{p{1cm} p{2cm} p{5cm}}
        \hline
        Simulator & Scopes  & Highlights \\
        \hline
        \hline
 %%%
 \CausalSim \cite{CausalSim} & the bias introduced by the choices of algorithms during trace collection & \begin{itemize}
     \item Uses causal models to understand underlying system conditions
     \item Begins with an randomized control trial (RCT) to debias data for new algorithm simulation
     \item Maps simulation to a tensor completion problem, effective even with sparse data
 \end{itemize}\\
 \hline
 \SUMOITS \cite{SUMO2018} & intelligent transportation system, traffic simulation & \begin{itemize}
    \item Capable of handling complex networks and dense traffic scenarios.
    \item each vehicle has an own route, and moves individually through the road network.
    \item Supports plugins and external application programming interfaces (APIs), allowing integration with other software.
    \item Simulates various models of transportation.
 \end{itemize}\\
 \hline
 \SimMobility \cite{simmobility} & intelligent transportation system, mobility simulation & \begin{itemize}
    \item Covers long-term (urban planning), medium-term (transport demand), and short-term (real-time traffic flows) aspects.
    \item Capable of incorporating models from economics, sociology, and other disciplines to study the complex impacts of different policies.
    \item Particularly useful for policy analysis and urban planning, focusing on sustainable development and socio-economic impact analyses.
 \end{itemize} \\
%%%
 \SLEIPNIR \cite{sleipnir} & mobile cloud/edge/iot computing & a DAG scheduling simulator \\
 \hline

    \end{tabular}
    \begin{minipage}{16cm}
        \smallskip
        \textsuperscript{1}xxx \\
        \textsuperscript{2}yyy
    \end{minipage}
\end{table}


